A Declarative Modelling Framework for the Deployment and Management of Blockchain Applications

The deployment and management of Blockchain applications require non-trivial efforts given the unique characteristics of their infrastructure (i.e., immutability) and the complexity of the software systems being executed. The operation of Blockchain applications is still based on ad-hoc solutions that are error-prone, difficult to maintain and evolve, and do not manage their interactions with other infrastructures (e.g., a Cloud backend). This paper proposes KATENA, a framework for the deployment and management of Blockchain applications. In particular, it focuses on applications that are compatible with Ethereum, a popular general-purpose Blockchain technology. KATENA provides i) a metamodel for defining Blockchain applications, ii) a set of processes to automate the deployment and management of defined models, and iii) an implementation of the approach based on TOSCA, a standard language for Infrastructure-as-Code, and xOpera, a TOSCA-compatible orchestrator. To evaluate the approach, we applied KATENA to model and deploy three real-world Blockchain applications, and showed that our solution reduces the amount of code required for their operations up to $82.7\%$.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> sections/implementation-2.tex <==

Two example scenarios that illustrates the prototype in action are shown in Figures \ref{fig:implementation:deploy-Library} and \ref{fig:implementation:Diamond-destroy}. Since both of them require some common, preliminary operations, that is, the setup of wallet and network nodes, they are discussed once and then omitted for brevity. 

\textbf{Preliminary operations.} Each \approach file must define two essential TOSCA nodes that enable the interaction with the Blockchain: a wallet and a network. When xOpera starts processing the TOSCA components defined in the file, these two nodes are the first ones it creates since they do not have any requirements specified.
The network node checks the reachability of the Blockchain endpoint while the wallet takes the address and private key of the Blockchain wallet, which are safely stored in a separated file on the local device. \luc{E cosa ci facciamo?}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{images/tosca-deploy-workflow.pdf}
    \caption{Library linkage and smart contract dependencies.}
    \label{fig:implementation:deploy-Library}
\end{figure}

\textbf{Libraries and smart contracts.}
Figure \ref{fig:implementation:deploy-Library} shows an example deployment of a simple application that includes a library and three smart contracts. The dependency graph is represented in the top part of the figure by means of arrows and two grey boxes highlight the main interactions implemented by \approach.

Box $1$ covers the Library linkage between smart contract \textit{Smart Contract 1} and \textit{Library}.  Smart contract \luc{Node: di cosa stiamo parlando?} has a contract-library dependency defined as \textit{Library: L} \luc{Dove lo vedo?} in the requirement field and so the deployment starts with L. \luc{Ma L non \`e un elemento del diagramma. O cambiamo il diagramma o il testo: non credo che un minimo di consistenza sia cos\`i difficile}

Since \luc{L} has no library-library dependencies, it is deployed with no extra operations. \luc{A reference to it} is saved in its attribute  \textit{address}. Then we focus on \luc{C1}, 
and we run the script in charge of substituting placeholders with library references. The script is linked to the \luc{useLibrary} association and, to ensure its correct execution, is invoked when the TARGET of the relationship \luc{quale? Qui credo si stia parlando di TOSCA, ma sopra del nostro meta-modello. Sbaglio?} (i.e., the library) has finished the deployment.

Box $2$ shows how lazy-contract-contract and contract-contract dependencies are handled. The dependency between smart contract \textit{C1} and smart contract 2 \textit{C2} \luc{Continuo a dire che i nomi in figura sono diversi} is managed by the call association. As previously stated in Section \ref{fig:solution:metamodel}, this association implies the invocation of a specific function after deploying the smart contract \luc{Quale?}. So, the deployment of \luc{C1 and C2} can proceed independently and then the function to set the address can be called. \luc{Non ho capito. Quale funzione? \`e la funzione specifica di cui sopra?} 

In contrast, the contract-contract dependency between \luc{C1} and \luc{smart contract 3 \textit{C3}} requires a different approach since the reference to \luc{C1} is passed as parameter to \luc{C3}'s constructor. The prototype retrieves the reference to \luc{C1} by means of the \textit{CallsInConstructor} requirement \luc{Da dove salta fuori? \\`E TOSCA o metamodello? Perch\'e requirement?}. All collected references need to be merged with parameter properties where users specify other parameters, if any \luc{Cosa vuol dire la frase precedente? Perch\'e parliamo di tutti gli indirizzi/riferimento che \`e uno solo? Quali parametri?}. To achieve this, we implemented a dedicated ABI parser for Solidity versions 0.5.x and 0.8.x. \luc{Perch\'e ci serve un parser dedicato per ABI per fare il merge di parametri? Da dove salta fuori Solidity? Perch\'e dobbiamo specificare le due versioni?} The parser takes the list of references \luc{Sempre una nell'esempio, credo} and parameters \luc{quali nell'esempio. Ci sono?} and parses the signature of the smart contract's constructor \luc{Quale?} and merges the two lists to fit the signature. \luc{Perch\'e server un parser per fare il merge di due eventuali liste?}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.735\linewidth]{images/tosca-diamond-workflow.pdf}
    \caption{Deployment of a diamond-based contract.}
    \label{fig:implementation:Diamond-destroy}
\end{figure}

\luc{Non ho capito. Alla fine, le uniche due cose che fa il prototipo \`e risolvere un paio di dipendenze? O lo diciamo molto male, oppure mi sembra azzardato chiamarlo protitpo. Se tutto il lavoro si riassume veramente in Figura 4, forse vale la pena ritirare l'abstract e l'articolo.}

\subsection{Example scenario}

\luc{come sempre mi sembra una sotto-sezione molto breve}

Figure \ref{fig:implementation:Diamond-destroy} presents an example scenario to show how the prototype works. \luc{Non ho capito la differenza con figura 4} \luc{Faccio notare che se sono sequence diagram, e non vogliamo inventarci notazioni, le entit\`a dovrebbero essere dei rettangoli, ma le operazioni no. Dovrebbero essere delle annotazioni agli archi/linee tra oggetti} \luc{Aggiungo che \`e ovvio che il tempo vada dall'alto in basso. Si insegna in Ingegneria del Sw 1}

The prototype is used to instantiate a diamond-based contract \luc{Credo si voglia istanziare un contratto} within a smart contract destruction scenario \luc{Cosa \`e uno smart contract destruction scenario?}. The scenario comprises three elements: a \textit{Facet}, a \textit{DiamondCut}, and a \textit{Diamond}. \luc{Non capisco perch\'e si debbano chiamare D, DC e F quando nella figura hanno nomi diversi}

\textit{Step 2. Diamond composition.} \luc{Toglierei tutto il titolo, ma partire dal passo 1 ci sembrava riduttivo?} The box \luc{Toglierei il numero in figura, visto che \`e uno solo} shows the deployment of a Diamond design pattern instance. \luc{Ma non lo abbiamo appena detto sopra?} We first deploy the facet \luc{F} and the diamondCut \luc{DC}. We then retrieve the reference to \luc{DC}, thanks to the \textit{callInConstructor} relationship specified in the \textit{cut} requirement \luc{cut requirement?} and pass it to the diamond's while deploying it. After that, the \textit{useFacet} relationship triggers the execution of a script which calls the diamondCut function \luc{Ma diamondCut non \`e una funzione} and adds F functions. \luc{Quali funzioni, quali F, a cosa?}

Note that , the DiamondInit Facet is modelled but not fully implemented \luc{in effetti, i due sequence diagram sono gi\`a troppo complicati}. While this does not compromise the usability of the approach, its implementation is left for future work in which we aim to elicit the set of known design patterns for smart-contract applications and apply them comparatively in the scope of controlled experimentation. \luc{Mi sembra che la frase finale non serva nulla e ci faccia solo male. Se c'\`e c\`e e se non c'\`e, non c'\`e, ai lavori futuri ci penseremo poi.}

\luc{Ammetto che io non ho ancora capito a cosa serva TOSCA qui, rispetto al nostro meta-modello, cosa faccia xOpera e cosa faccia effettivamente il nostro prototipo. I due semi sequence diagram mi sembrano abbastanza ovvi. No? Serve un nuovo approccio ed un prototipo innovativo per farli?}

==> sections/problem-statement.tex <==
% \section{problem statement}\label{sec:problem-statement} 
% A dApp is composed by a set of contracts that interacts with each other and so, they have dependencies that must be satisfied. 
% % - gestione degli address error prone in script imperativi
% As the size in terms of contracts of the decentralized applications keeps growing, the number of addresses to track is increasing. This makes the deployment scripts more complicated to write, maintain and debug \lt{credo si debba stare attenti a questa frase}.

% % - dipendenze per deployment
% % "on chain components with internal dependencies
% In particular, as stated in Section \ref{sec:background}, a contract needs the memory address of another one to being able to contact it. This kind of constraint forms a chain of dependencies between the application smart contracts that affects the application deployment.
% In fact, the memory address is not known a-priori but only once the smart contract is deployed to the Blockchain. This enforces users to deploy some contracts before others in order to have all the required data to instatiate them.

% % - runtime update peggiora il tutto
% Upgradeable smart contracts introduce the runtime management of the dApp. They enable developers to change at the implementation of a contract once it has been deployed. To cope with this behavior, dedicated script needs to be made to update the relevant part of the infrastructure

% % When users wants to deploy a decentralized application, what they need to do first is to retrieve an endpoint to communicate with the Blockchain network that will host the application. As stated in Section \ref{sec:balancing}

% % "on chain components with external dependency 
% % (dApp comunicano sempre di piu' tra loro)"
% % off chain components
% % "A declarative approach does not exist
% % (need cite from comparison with cloud)"


% % problemi:



